A Survey on Test-Time Scaling in Large Language Models: What, How, Where, and How Well?

As enthusiasm for scaling computation (data and parameters) in the pretraining era gradually diminished, test-time scaling (TTS), also referred to as ``test-time computing'' has emerged as a prominent research focus. Recent studies demonstrate that TTS can further elicit the problem-solving capabilities of large language models (LLMs), enabling significant breakthroughs not only in specialized reasoning tasks, such as mathematics and coding, but also in general tasks like open-ended Q&A. However, despite the explosion of recent efforts in this area, there remains an urgent need for a comprehensive survey offering a systemic understanding. To fill this gap, we propose a unified, multidimensional framework structured along four core dimensions of TTS research: what to scale, how to scale, where to scale, and how well to scale. Building upon this taxonomy, we conduct an extensive review of methods, application scenarios, and assessment aspects, and present an organized decomposition that highlights the unique functional roles of individual techniques within the broader TTS landscape. From this analysis, we distill the major developmental trajectories of TTS to date and offer hands-on guidelines for practical deployment. Furthermore, we identify several open challenges and offer insights into promising future directions, including further scaling, clarifying the functional essence of techniques, generalizing to more tasks, and more attributions. Our repository is available on https://github.com/testtimescaling/testtimescaling.github.io/

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> section/fig.tex <==
\tikzstyle{my-box}= [
    rectangle,
    draw=hidden-draw,
    rounded corners,
    text opacity=1,
    minimum height=1.5em,
    minimum width=5em,
    inner sep=2pt,
    align=center,
    fill opacity=.5,
]
\tikzstyle{leaf}=[my-box, minimum height=1.5em,
    fill=orange!60, text=black, align=left,font=\scriptsize,
    inner xsep=2pt,
    inner ysep
=4pt,
]
\begin{figure}[!htbp]
\vspace{-2.5em}
\centering
% \resizebox{\textwidth}{!}{
\scalebox{0.7}{
    \begin{forest}
        forked edges,
        for tree={
            grow=east,
            reversed=true,
            anchor=base west,
            parent anchor=east,
            child anchor=west,
            base=left,
            font=\small,
            rectangle,
            draw=hidden-orange,
            rounded corners,
            align=left,
            minimum width=4em,
            edge+={darkgray, line width=1pt},
            s sep=3pt,
            inner xsep=2pt,
            inner ysep=3pt,
            ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
        },
            where level=1{text width=4.5em,font=\scriptsize,}{},
            where level=2{text width=5.4em,font=\scriptsize,}{},
            where level=3{text width=6.4em,font=\scriptsize,}{},
            where level=4{text width=6.4em,font=\scriptsize,}{},
[
    \textbf{Test-time Scaling}, ver
    [
        \textbf{What to Scale}\\ (\S \ref{sec:what2scale})
        [
            \textbf{Parallel Scaling} \\ (\S \ref{subsec:parallelsclaing})
            [
                Self-Consistency~\citep{brown2024largelanguagemonkeysscaling, irvine2023rewarding, song2024good, snell2024scaling, wang2023selfconsistency, nguyen2024consistent} \\ 
                \citep{chen2024are, wu2025lessunderstandingchainofthoughtlength}{,} 
                Multi-Agents~\citep{jiang2023llm}{,}
                PlanSearch~\citep{wang2024planningnaturallanguageimproves}{,}
                CCE~\citep{zhang2025crowd}, leaf, text width=40em
            ]
        ]
        [
            \textbf{Sequential Scaling}\\ (\S \ref{subsec:sequentialsclaing})
            [
                Self-Refine~\citep{madaan2023selfrefine, chen2024teaching, gou2024critic, zhang2024smalllanguagemodelsneed}{,}
                Sequential Revision~\citep{lee2025evolvingdeeperllmthinking}{,} ReAct\\
                \citep{yao2023react}{,}
                Budget-aware~\citep{kimi-k1.5, muennighoff2025s1, han2025tokenbudgetawarellmreasoning}{, }RecurrentBlock~\citep{geiping2025scalingtesttimecomputelatent}{,} STaR\\
                \citep{yuan2023scaling, singh2024beyond}{,} 
                Meta-STaR~\citep{xiang20252reasoningllmslearning}{,}
                PlanningToken~\citep{wang2024guiding}{,}
                RaLU~\citep{li2025reasoningaslogicunitsscalingtesttimereasoning}, leaf, text width=40em
            ]
        ]
        [
            \textbf{Hybrid Scaling}\\ (\S \ref{subsec:hybridsclaing})
            [
                MoA~\citep{wang2025mixtureofagents}{,}
                Tree of Thoughts~\citep{yao2023tree, zhang2024chain}{,}
                Graph of Thoughts~\citep{Besta2024graph}{,} Tree-Search\\
                \citep{chen2024tree}{,} 
                SoS~\citep{gandhi2024streams}{,}
                REBASE~\citep{wu2024scaling}{,} 
                OAIF~\citep{guo2024direct}{,}
                Beam-Search~\citep{guo2024direct}{,}M-\\
                CTS\citep{tian2024toward, zhang2024o1coder, gao2024interpretable, wan2024alphazero, chenalphamath}{,} 
                Journey Learning\citep{GAIR-o1p1}{,}A-\\
                daptiveAlloc\citep{snell2024scaling, ong2025routellm}{,}
                METAL\citep{li2025metalmultiagentframeworkchart}{,}
                rStar-Math\citep{guan2025rstarmathsmallllmsmaster}{,}AtomThink\citep{xiang2024atomthinkslowthinkingframework}, leaf, text width=40em
            ]
        ]
        [
            \textbf{Internal Scaling}\\ (\S \ref{subsec:internalsclaing})
            [
                DeepSeek-R1~\citep{deepseek-r1}{,}
                OpenAI-o1\&o3~\citep{openai-o1,openai-o3}{,}
                Gemini Flash Thinking~\citep{geminithinking}{,}
                QwQ~\citep{qwq-32b-preview}{,}\\
                K1.5~\citep{kimi-k1.5}{,}
                3SUM~\citep{pfau2024lets}{,}
                OAIF~\citep{guo2024direct}{,}
                LIMO~\citep{ye2025limoreasoning}{,}
                 T1~\citep{hou2025advancing}{,}
                Distilled-o1\\~\citep{GAIR-o1p2}{,}
                RedStar~\citep{xu2025redstardoesscalinglongcot}{,}
                SKY-T1~\citep{skyt12025}{,}s1~\citep{muennighoff2025s1}{,} ITT~\citep{hao2024training}, leaf, text width=40em
            ]
        ]
    ]
    [
        \textbf{How to Scale} \\ (\S \ref{sec:how2scale})
        [
            \textbf{Tuning} (\S \ref{subsec:tuning})
            [
                \textbf{Supervised} \\ \textbf{Finetuning} (\S \ref{subsubsec:sft})
                [
                    Distillation~\citep{muennighoff2025s1, GAIR-o1p2, xu2025redstardoesscalinglongcot, skyt12025, bespoke_stratos} \\
                    \citep{munkhbat2025selftrainingelicitsconcisereasoning, ye2025limoreasoning}{,}  
                    Synthesized Long CoT~\citep{hou2025advancing, yeo2025demystifying}{,} \\
                    Learning Reasoning Structure~\citep{li2025llmseasilylearnreason}{,} 
                    Long CoT warmup~\citep{kimi-k1.5}{ ,}
                    CFT~\citep{wang2025critiquefinetuninglearningcritique}, leaf, text width=32em 
                ]
            ]
            [
                \textbf{Reinforcement}\\ \textbf{Learning} (\S \ref{subsubsec:rl})
                [
                    \textbf{Reward model-free}
                    [
                        Rule-Based~\citep{deepseek-r1}{,}
                        cDPO~\citep{lin2024critical}{,}
                        Focused-DPO\\
                        \citep{zhang2025focused}{,}
                        Selective DPO~\citep{gao2025principled}{,}
                        CPL~\citep{wang2024cpl}{,} \\
                        OREO~\citep{wang2024offline}{,} 
                        DAPO~\citep{liu2024improvingmultistepreasoningabilities}{,}
                        RFTT~\citep{zhang2025reasoning}{,} \\
                        SimPO~\citep{meng2024simpo}{,} 
                        DQO~\citep{ji2024enhancing}{,}
                        DAPO~\citep{yu2025dapo}{,} \\
                        VC-PPO~\citep{yuan2025s}{,} 
                        Light-R1~\citep{wen2025lightxi}{,} \textit{etc.}, leaf, text width=24em
                    ]
                ]
                [   
                    \textbf{Reward model-based}
                    [
                        PPO~\citep{schulman2017proximalpolicyoptimizationalgorithms}{,}
                        RLOO~\citep{ahmadian2024back}{,} \\
                        GRPO~\citep{shao2024deepseekmath}{,} 
                        REINFORCE++~\citep{hu2025reinforce++}{,}
                        DVPO~\citep{huang2025lean}{,} \\
                        PRIME~\citep{cui2025process}{,} 
                        SPPD~\citep{yi2025sppd}{,} \textit{etc.}, leaf, text width=24em
                    ]
                ]
                % [
                %     Optimization Policy
                %     [
                %         GRPO~\citep{deepseek-r1, deepseek-math}{,}
                %         PPO~\citep{schulman2017proximalpolicyoptimizationalgorithms}{,} \\
                %         OPMD (variant)~\citep{kimi-k1.5}{,}
                %         DPO~\citep{zhang2024chain, NEURIPS2023_a85b405e}{,} \\
                %         OPMD~\citep{pmlrlazic19a, tomar2021mirrordescentpolicyoptimization}{,}DAPO~\citep{liu2024improvingmultistepreasoningabilities}, leaf, text width=24em
                %     ]
                % ]
                % [
                %     \textbf{Reward Modeling}
                %     [
                %         Rule-Based~\citep{deepseek-r1}{,}
                %         Classic~\citep{ouyang2022training}{,} Generative-RM\\\citep{mahan2024generativerewardmodels}{,}LLM-as-a-Judge\citep{guo2024direct}{,}DVPO~\citep{huang2025lean}{,}\\
                %         Multi-RM\citep{gao2024interpretable}{,}
                %         RLOO\citep{ahmadian2024back}{,}PUP\citep{hou2025advancing}{,}\\
                %         PRM\citep{wang-etal-2024-math}{,}PRIME\citep{cui2025process}{,}GLoRe~\citep{havrilla2024glorewhenwhereimprove}{,}
                %         , leaf, text width=24em
                %         %CoT\citep{ankner2024critiqueoutloudrewardmodels, kimi-k1.5}{, }
                %     ]
                % ]
            ]
        ]
        [
            \textbf{Inference} (\S \ref{subsec:inference})
            [
                \textbf{Stimulation} (\S \ref{subsec:stimulation})
                [
                    \textbf{Prompt Strategy} % \\ (\S \ref{Tuning})
                    [
                        Hint-infer~\citep{li2025startselftaughtreasonertools}{,}                        Dipper~\citep{lau2024dipperdiversitypromptsproducing}{,}
                        EVA~\citep{ye2024evolvingalignmentasymmetricselfplay}{,} 
                        \\EvalPlan\citep{saha2025learningplanreason}{,} 
                        ReasonFlux~\citep{yang2025reasonflux}{,}~\citet{10460413}
                        , leaf, text width=24em
                    ]
                ]
                [
                    \textbf{Decode Strategy} % \\ (\S \ref{Tuning})
                    [
                        Filler Tokens~\citep{pfau2024lets}{,}
                        Budget Forcing~\citep{muennighoff2025s1}{,} LTV\\
                        \citep{kong2025scalablelanguagemodelsposterior}{,}
                        AFT~\citep{li2025draftsanswersunlockingllm}{,} 
                        Predictive-Decoding~\citep{ma2025nonmyopic},leaf, text width=24em
                        %Adaptive Injection~\citep{jin2025wellthinkingenhancingllm},
                    ]
                ]
                [
                    \textbf{Self-Repetition}
                    [
                        Self-Consistency~\citep{wang2023selfconsistency}{,}
                        Self-Refine~\citep{madaan2023selfrefine}{,} DeCRIM\\
                        \citep{ferraz2024llmselfcorrectiondecrimdecompose}{,} CCE~\citep{zhang2025crowd}{,}
                        TreeBoN~\citep{qiu2024treebonenhancinginferencetimealignment}, leaf, text width=24em
                    ]
                ]
                [
                    \textbf{Mixture-of-Model}
                    [   
                        MoA~\citep{wang2025mixtureofagents}{,}
                        RR-MP~\citep{he2025enhancingllmreasoningmultipath}{,}
                        BRAIN~\citep{chen2024braininspiredtwostageapproachenhancing}, leaf, text width=24em
                    ]
                ]
            ]
            [
                \textbf{Verification} (\S \ref{subsec:verification})
                [
                    \textbf{Outcome}
                    [
                        Output Verification~\citep{cobbe2021training}{,} Generative Verifier~\citep{zhang2025generativeverifiersrewardmodeling}{,}\\Self-Reflection Feedback~\citep{li2025learningreasonfeedbacktesttime}{,} Discriminator~\citep{chen2024tree}{,}\\
                        OVM~\citep{yu2024ovm}{,} Heuristic~\citep{deepseek-r1}{,} Bandit~\citep{sui2025metareasonerdynamicguidanceoptimized}{,}\\
                        Functional~\citep{lee2025evolvingdeeperllmthinking}{,} 
                        XoT~\citep{liu2023plan}{,} 
                        WoT~\citep{zhang2024wrongofthoughtintegratedreasoningframework}, leaf, text width=24em
                    ]
                ]
                [
                    \textbf{Process}
                    [
                        State Evaluator~\citep{yao2023tree,zhang2024chain}{,}
                        SIaM~\citep{yu2024siamselfimprovingcodeassistedmathematical}{,}\\
                        Deductive Verification~\citep{ling2023deductive}{,}
                        Self-Evaluator~\citep{xie2023selfevaluation}{,} \\
                        V-STaR~\citep{hosseini2024vstartrainingverifiersselftaught}{,}
                        Tool~\citep{li2025startselftaughtreasonertools}{,}
                        PoT~\citep{chen2023program}, leaf, text width=24em
                    ]
                ]
                %[
                %    Multi-Criteria
                %    [
                %        {,} 
                %        MAV~\citep{lifshitz2025multiagent}, leaf, text width=24em
                %    ]
                %]
            ]
            [
                \textbf{Search} (\S \ref{subsec:search})
                [
                    TreeSearch~\citep{yao2023tree,chen2024tree}{,}GraphSearch~\citep{Besta2024graph}{,}C-MSTS~\citep{lin2025leveragingconstrainedmontecarlo}{,}\\
                    MCTS~\citep{tian2024toward,zhang2024o1coder,gao2024interpretable, wan2024alphazero,chenalphamath}{,} SPaR\\
                    \citep{cheng2025sparselfplaytreesearchrefinement}{,}
                    REBASE~\citep{wu2024scaling}{,}
                    SoS~\citep{gandhi2024streams}{,} CoAT~\citep{pan2025coatchainofassociatedthoughtsframeworkenhancing}{,}Beam-\\
                    Search~\citep{guo2024direct,xie2023selfevaluation}{,}
                    Lookahead-Search~\citep{snell2024scaling, zhang2023planning}{,}\textit{ etc.}, leaf, text width=32em
                    %DVTS~\citep{beenching2024scaling}{,} \\
                    % S*~\citep{li2025stesttimescaling}{,}\\
                    %Seed-CTS~\citep{wang2024seedctsunleashingpowertree}{,}%BRiTE~\citep{zhong2025britebootstrappingreinforcedthinking}{,}
                    %NGS~\citep{kim2025neuralgeneticsearchdiscrete},leaf
                ]
            ]
            [
                \textbf{Aggregation} (\S \ref{subsec:aggregation})
                % [
                %     Best-of-N~\citep{brown2024largelanguagemonkeysscaling, irvine2023rewarding, song2024good, li2023making}{,}\\
                %     Majority Voting~\citep{wang2023selfconsistency,nguyen2024consistent,chen2024are}{,}
                %     AFT~\citep{li2025draftsanswersunlockingllm}{,}\\
                %     Length-filtered Vote~\citep{wu2025lessunderstandingchainofthoughtlength}{,}
                %     Few-shot Sampling~\citep{munkhbat2025selftrainingelicitsconcisereasoning}{,}
                %     Rejection Sampling\\\citep{kimi-k1.5}{,} 
                %     Routation~\citep{ong2025routellm}{,}
                %     % Journey Learning~\citep{GAIR-o1p1}{,}
                %     Filter-Vote~\citep{chen2024are}{,}\\ 
                %     % WoT~\citep{zhang2024wrongofthoughtintegratedreasoningframework}{,}
                %     Synthesize~\citep{wang2025mixtureofagents}{,} 
                %     PairRanker~\citep{jiang2023llm}{,} \\
                %     GSA~\citep{li2025llmsgeneratebetteranswer}{,}
                %     BOND~\citep{sessa2024bondaligningllmsbestofn}, leaf, text width=32em
                % ]
                [
                    \textbf{Selection}
                    [
                        Majority Voting\citep{wang2023selfconsistency, chen2024are}{,} BOND\citep{sessa2024bondaligningllmsbestofn}{,}\\
                        Filter Vote\citep{chen2024are}{,} 
                        Length-filtered Vote\citep{wu2025lessunderstandingchainofthoughtlength}{,} Best-of-N\\
                        \citep{irvine2023rewarding, song2024good}{,} Rejection Sampling~\citep{kimi-k1.5}{,} \textit{etc.} 
                        %FS-BoN~\citep{munkhbat2025selftrainingelicitsconcisereasoning}{,}
                        , leaf, text width=24em
                    ]
                ]
                [
                    \textbf{Fusion}
                    [
                        BoN (weighted)~\citep{brown2024largelanguagemonkeysscaling}{,} Synthesize~\citep{wang2025mixtureofagents}{,} \textit{etc.}, leaf, text width=24em
                    ]
                ]
            ]
        ]
    ]
    [
        \textbf{Where to Scale} \\ (\S \ref{sec:where2scale})
        [
            \textbf{Reasoning} (\S \ref{sec:reasoning})
            [
                \textbf{Math}
                [
                    AIME~\citep{aime25, guan2025rstar}{,}
                    CNMO~\citep{cnmo}{,}
                    NuminaMATH~\citep{numina_math_datasets}{,} OmniMath\\
                    \citep{gao2025omnimath}{,}
                    MATH~\citep{cobbe2021training, hendrycks2021measuring,guan2025rstar}{,} s1-prob-teasers\\
                    \citep{muennighoff2025s1}{,} 
                    GSM8K~\citep{guan2025rstar,zhang2024rest}{,} MATH500\citep{zhang2024rest}{,}\\
                    AMC~\citep{guan2025rstar}{,}
                    College Math~\citep{guan2025rstar}{,}
                    %CHMath~\citep{chmath}{,}
                    FrontierMath~\citep{glazer2024frontiermath}{,}\textit{ etc.}, leaf, text width=32em
                ]
            ]
            [
                \textbf{Code}
                [
                    USACO~\citep{shi2024can}{,}
                    LiveCodeBench~\citep{jain2025livecodebench}{,}
                    CodeContests~\citep{Li2022competition}{,} Aider-Polyglot\\
                    \citep{aider}{,}SWE-bench\citep{jimenez2024swebench}{,}Codeforces\citep{codeforce}{,}CodeMind~\citep{liu2024codemindframeworkchallengelarge}{,}\textit{ etc.}
                    , leaf, text width=32em
                ]
            ]
            [
                \textbf{Science}
                [
                    OlympicArena~\citep{huang2024olympicarena}{,}
                    OlympiadBench~\citep{he2024olympiadbench, guan2025rstar}{,} TheoremQA\\
                    \citep{chen2023theoremqa}{,}
                    JEEBench~\citep{arora2023have}{,}    
                    GPQA~\citep{rein2024gpqa}{,}
                    SciEval~\citep{sun2024scieval}{,}\\
                    Miverva~\citep{lewkowycz2022solving}{,}
                    SciBench~\citep{zhang2024rest}{,} HLE~\citep{phan2025humanity}{,}\textit{ etc.}\\
                    , leaf, text width=32em
                ]
            ]
            [
                \textbf{Game \& Strategy}
                [
                    SysBench~\citep{aime25}{,} Points24~\citep{yao2023tree,zhai2024finetuninglargevisionlanguagemodels}{,} TravelPlan~\citep{xie2024travelplannerbenchmarkrealworldplanning}{,}\textit{ etc.}, leaf, text width=32em
                ]
            ]
            [
                \textbf{Medical}
                [
                    SysBench{,} JMLE-2024~\citep{nori2024medprompt}{,}Medbullets~\citep{chen2025benchmarkinglargelanguagemodels}{,}MedQA~\citep{jin2020diseasedoespatienthave}{,}\textit{ etc.}, leaf, text width=32em
                ]
            ]
        ]
        [   
            \textbf{General-Purpose} \\ (\S \ref{sec:generalpurpose})
            [
                \textbf{Basics}
                [
                    AGIEval~\citep{zhong2024agieval}{,} 
                    MMLU-Pro~\citep{wang2024mmlupro}{,}  
                    Gaokao~\citep{gaokao, guan2025rstar}{,}\\
                    Kaoyan~\citep{kaoyan}{,} CMMLU~\citep{li2024cmmlumeasuringmassivemultitask}{,} LongBench~\citep{bai2024longbenchbilingualmultitaskbenchmark}{,} ARC-AGI~\citep{chollet2019measureintelligence}{,}\textit{ etc.}, leaf, text width=32em
                ]
            ]
            [
                \textbf{Agents}
                [
                    WebShop~\citep{yao2023webshop}{,} 
                    WebArena~\citep{zhou2023webarena}{,} 
                    SciWorld~\citep{wang2022sciworld}{,} 
                    WebVoyager\\
                    \citep{he2024webvoyagerbuildingendtoendweb}{,} TextCraft\citep{prasad2024adaptasneededdecompositionplanning}{,} TAU-bench~\citep{yao2024taubenchbenchmarktoolagentuserinteraction}{,} BCFL~\citep{berkeley-function-calling-leaderboard}{,}\textit{ etc.}, leaf, text width=32em
                ]
            ]
            [
                \textbf{Knowledge}
                [
                    SimpleQA~\citep{wei2024measuringshortformfactualitylarge}{,} 
                    C-SimpleQA~\citep{he2024chinesesimpleqachinesefactuality}){,}FRAMES~\citep{krishna2025factfetchreasonunified}{,}\textit{ etc.}, leaf, text width=32em
                ]
            ]
            [
                \textbf{Open-Ended}
                [
                    AlpacaEval2.0~\citep{dubois2024lengthcontrolledalpacaevalsimpleway}{,} 
                    ArenaHard~\citep{li2024crowdsourceddatahighqualitybenchmarks}{,} 
                    IF-Eval~\citep{zhou2023instructionfollowing}{,} Chatbot Arena\\
                    \citep{zheng2023judgingllmasajudgemtbenchchatbot}{,}
                    C-Eval~\citep{huang2023ceval}{,} FollowBench~\citep{jiang2024followbenchmultilevelfinegrainedconstraints}{,}\textit{ etc.}, leaf, text width=32em
                ]
            ]
            [
                \textbf{Multi-Modal}
                [
                    MMMU~\citep{yue2024mmmu}{,} 
                    MATH-Vision~\citep{wang2024measuring}{,}
                    MathVista~\citep{lu2024mathvista}{,} LLAVA-Wild\\
                    \citep{liu2023visual}{,}
                    MM-Vet~\citep{yu2024mm}{,}
                    MMBench~\citep{liu2024mmbench}{,}
                    MMMU~\citep{yue2024mmmu}{,} \\
                    CVBench~\citep{tong2024cambrian}{,}
                    MMStar~\citep{chen2024we}{,}
                    CHAIR~\citep{rohrbach2018object}{,}\textit{ etc.}, leaf, text width=32em
                ]
            ]
        ]
    ]
    [
        \textbf{How Well to}  \\ \textbf{Scale} (\S \ref{sec:howwell2scale})
        [
            \textbf{Accuracy} \\ (\S \ref{subsec:performance})
            [
               Pass@1\citep{deepseek-r1, kimi-k1.5}{, }Pass@k\citep{chen2021evaluating, brown2024large}{, }WinRate\citep{deepseek-r1, hou2025advancing}\\Cons@k~\citep{deepseek-r1, zeng2025revisiting}{, }{,}\textit{ etc.}, leaf, text width=40em
            ]
        ]
        [
            \textbf{Efficiency} \\ (\S \ref{subsec:efficiency})
            [
            Token Cost~\citep{welleck2024decoding, aytes2025sketchofthoughtefficientllmreasoning}{, }FLOPs-based Efficiency Analysis~\citep{kaplan2020scalinglawsneurallanguage, snell2024scaling}{, }KV Cache\\
            size~\citep{hooper2025etsefficienttreesearch}{, }
            Underthinking score~\citep{wang2025thoughtsplaceunderthinkingo1like}{,}
            \textit{ etc.}, 
               leaf, 
               text width=40em
            ]
        ]
        [
            \textbf{Controllability}\\ (\S \ref{subsec:controllability})
            [
               Control Metric~\citep{muennighoff2025s1}{,}Length Deviation~\citep{aggarwal2025l1}{,}$k$-$\epsilon$ Controllability~\citep{bhargava2024whatsmagicwordcontrol}{,}\textit{ etc.},  leaf, text width=40em
            ]
        ]
        [
            \textbf{Scalability}\\ (\S \ref{subsec:scalability})
            [
               Scaling Metric~\citep{muennighoff2025s1}{,}Scaling Curves (Accuracy vs. Compute)~\citep{aggarwal2025l1, teng2025atom}{,}\textit{ etc.}, leaf, text width=40em
            ]
        ]
    ]
]
\end{forest}
}
\vspace{-1em}
\caption{Taxonomy of research in Test-time Scaling that consists of what, how, where, and how well to scale.}
\label{categorization_of_reasoning}
\end{figure}

       % Token Cost~\citep{welleck2024decoding, aytes2025sketchofthoughtefficientllmreasoning}, 
            % FLOPs-based Efficiency Analysis~\citep{kaplan2020scalinglawsneurallanguage},
               % Dependency~\citep{bai2022constitutional}{,} 
               % Sample Efficiency~\citep{muennighoff2025s1,ye2025limoreasoning}{,} 
               % Scaling Efficiency (Length){,} \\
               % Difficulty~\citep{muennighoff2025s1, kimi-k1.5, ye2025limoreasoning}{,}
               % Diversity~\citep{muennighoff2025s1, kimi-k1.5, ye2025limoreasoning}{,} \\ 
               % Quality,
